Proximally Guided Stochastic Subgradient Method for Nonsmooth, Nonconvex Problems

In this paper, we introduce a stochastic projected subgradient method for weakly convex (i.e., uniformly prox-regular) nonsmooth, nonconvex functions---a wide class of functions which includes the additive and convex composite classes. At a high-level, the method is an inexact proximal point iteration in which the strongly convex proximal subproblems are quickly solved with a specialized stochastic projected subgradient method. The primary contribution of this paper is a simple proof that the proposed algorithm converges at the same rate as the stochastic gradient method for smooth nonconvex problems. This result appears to be the first convergence rate analysis of a stochastic (or even deterministic) subgradient method for the class of weakly convex functions.

==> conclusion.tex <==
\section{Conclusion}

In this paper we introduced a stochastic projected subgradient method for finding stationary points of weakly convex functions---a wide class of functions which includes additive and convex composite minimization problems. We provided a simple proof that, under mild assumptions, the algorithm converges at the same rate as the stochastic gradient method for smooth minimization problems. %For extremely large-scale finite sum problems, the proposed method performs on par with specialized optimization methods, while, in some cases, being simpler to implement.
